Minimising virtual machine support for concurrency

Co-operative and pre-emptive scheduling are usually considered to be complementary models of threading. In the case of virtual machines, we show that they can be unified using a single concept, the bounded execution of a thread of control, essentially providing a first-class representation of a computation as it is reduced. Furthermore this technique can be used to surface the thread scheduler of a language into the language itself, allowing programs to provide their own schedulers without any additional support in the virtual machine, and allowing the same virtual machine to support different thread models simultaneously and without re-compilation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{135}
\providecommand{\publicationstatus}{N. Yoshida, W. Vanderbauwhede (Eds.): Programming Language\\ Approaches to Concurrency- and Communication-cEntric\\Software 2013 (PLACES'13)\\
EPTCS 137, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.137.11}{10.4204/EPTCS.137.11}}

